MoonGS: High-quality Representation of the Lunar Surface via Gaussian Splatting Using Robust Depth Features from Image Pairs

High-quality 3D reconstruction of lunar terrain from sparse rover images is indispensable for autonomous lunar exploration, but remains challenging because viewpoint overlap is insufficient, surface textures are weak, and data volume is limited. We propose MoonGS, the first feed-forward 3D Gaussian Splatting framework tailored to lunar scenes. Given only two input images, MoonGS predicts pixel-aligned Gaussian primitives in a single forward pass and renders photorealistic novel views without any per-scene optimization. MoonGS (i) adopts an adaptable backbone design that seamlessly integrates advanced vision foundation models to extract robust depth features; (ii) integrates semantic priors in two manners: merging semantic cues with visual features to refine Gaussian parameter estimation, and adopting a semantic ranking loss that regularizes background depth; and (iii) employs an entropy-guided heuristic resampling strategy to augment sparse observations by selecting the most informative distant viewpoints with negligible overhead. Experiments on the LuSNAR benchmark and our synthetic weak-texture MoonBlender dataset show that MoonGS surpasses state-of-the-art feed-forward NeRF/3DGS baselines by +4.9 dB PSNR, +0.29 SSIM, and 40\% lower LPIPS while maintaining sub-second inference. Furthermore, we validate the broad applicability of our framework by demonstrating that it effectively leverages state-of-the-art backbones, including VGGT, to significantly boost performance. Qualitative evaluations on Chang'e mission imagery also show the best visual quality among compared methods, indicating robustness on real lunar data. The source code and dataset are publicly available at https://github.com/InRobots/MoonBlender.

==> figs/ablation_resample_strategy/ablation_resample_strategy.tex <==
\begin{figure}[hbtp]
    % \vspace{-1em}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/ablation_resample_strategy/ablation_resample_strategy_fig.pdf}
    \vspace{-5pt}
    \caption{\textbf{Ablation of heuristic resampling strategy.} 
    Our proposed strategy can, under a self-supervised setting without requiring manual intervention or prior knowledge, achieve performance comparable to the optimal results of a fixed-interval search.
    }
    \vspace{-15pt}
    \label{fig:ablation_resample_strategy}
\end{figure}

==> figs/change_percentage/joint.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/change_percentage/percentage_change.pdf}
    \vspace{-10pt}
    \caption{\textbf{Semantic pixel distribution for the LuSNAR and MoonBlender datasets.} Although MoonBlender contains fewer semantic categories than LuSNAR, it exhibits a higher proportion of weakly textured regions (e.g., the sky).}
    \label{fig:percentage}
    \vspace{-2em}
\end{figure}

==> figs/overall/small.tex <==
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{375bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.92490912)%
    \lineheight{0.1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{figs/overall/compare_all.pdf}}%
    % \put(0.05754546,0.90320912){\makebox(0,0)[t]{\lineheight{0.1}\smash{\begin{tabular}[t]{c}Ref.\end{tabular}}}}%
    % \put(0.22,0.90320912){\makebox(0,0)[t]{\lineheight{0.1}\smash{\begin{tabular}[t]{c}Target View\end{tabular}}}}%
    % \put(0.44,0.90320912){\makebox(0,0)[t]{\lineheight{0.1}\smash{\begin{tabular}[t]{c}Ours\end{tabular}}}}%
    % \put(0.670,0.90320912){\makebox(0,0)[t]{\lineheight{0.1}\smash{\begin{tabular}[t]{c}Pixelsplat~\cite{charatan2024pixelsplat}\end{tabular}}}}%
    % \put(0.895,0.90320912){\makebox(0,0)[t]{\lineheight{0.1}\smash{\begin{tabular}[t]{c}MVSplat~\cite{chen2025mvsplat}\end{tabular}}}}%
    % \put(0.90890912,0.91320912){\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}pixelNeRF~\cite{pixelnerf}\end{tabular}}}}%
  \end{picture}%
\endgroup%


==> figs/rank_loss/rank_loss.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/rank_loss/rankingloss2.pdf}
    \vspace{-10pt}
    \caption{\textbf{Ranking.} }
    \vspace{-15pt}
    \label{fig:ranking_loss}
\end{figure}

==> figs/rank_loss/ranking_loss2.tex <==
\begin{figure}[htp]
    \centering
    % Input Views
    % \begin{minipage}{0.1345\textwidth}
    % \caption*{Ref.}
    %     \includegraphics[width=\linewidth]{figs/rank_loss/minipage/pixelsplat.pdf}
        
    % \end{minipage}
    % \hfill
    \begin{minipage}{0.11\textwidth}
    \caption*{pixelSplat~\cite{charatan2024pixelsplat}}
        \includegraphics[width=\linewidth]{figs/rank_loss/minipage/pixelsplat.pdf}
        
    \end{minipage}
    % \hfill
    \begin{minipage}{0.11\textwidth}
    \caption*{MVSplat~\cite{chen2025mvsplat}}
        \includegraphics[width=\linewidth]{figs/rank_loss/minipage/mvsplat.pdf}
        
    \end{minipage}
    % \hfill
    \begin{minipage}{0.11\textwidth}
     \caption*{w/o Ranking}
        \includegraphics[width=\linewidth]{figs/rank_loss/minipage/worankingloss.pdf}
       
    \end{minipage}
    % \hfill
    \begin{minipage}{0.11\textwidth}
     \caption*{Ranking loss}
        \includegraphics[width=\linewidth]{figs/rank_loss/minipage/rankingloss.pdf}
       
    \end{minipage}
 \caption{
 \textbf{Comparison results about predicted depth maps.} Compared to 3DGS-based methods, our model using ranking loss has smoother depth maps in low-texture areas.
 % Comparison results about 3D Gaussians (top) and predicted depth maps of the reference viewpoints (bottom). Compared to SOTA 3DGS-based methods~\cite{charatan2023pixelsplat, chen2024mvsplat}, our method achieves higher quality in 3D Gaussian Splatting and produces smoother depth maps.
% 几何重建质量对比结果。第一列为输入的reference视角。相比于SOTA 3DGS-based methods，我们的方法重建3DGS的质量更高且depth map更平滑。
 }
	\label{fig:ranking_loss2}
 \end{figure}

==> figs/resource/resource.tex <==
\begin{figure}[hb]
    % \vspace{-1em}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/resource/cost.pdf}
    % \vspace{-5pt}
    \caption{\textbf{Effect of semantic downsampling.} The results depicted here show the influence of semantic downsampling on both image quality and memory consumption. The gray plane serves as the baseline, with all conventional methods yielding lower image quality compared to this reference. In contrast, semantic downsampling achieves a balance of acceptable image quality and reduced memory usage.}
    % \vspace{-1em}
    \label{fig:resource}
\end{figure}
